Selling to Multiple No-Regret Buyers

We consider the problem of repeatedly auctioning a single item to multiple i.i.d buyers who each use a no-regret learning algorithm to bid over time. In particular, we study the seller's optimal revenue, if they know that the buyers are no-regret learners (but only that their behavior satisfies some no-regret property -- they do not know the precise algorithm/heuristic used). Our main result designs an auction that extracts revenue equal to the full expected welfare whenever the buyers are "mean-based" (a property satisfied by standard no-regret learning algorithms such as Multiplicative Weights, Follow-the-Perturbed-Leader, etc.). This extends a main result of [BMSW18] which held only for a single buyer. Our other results consider the case when buyers are mean-based but never overbid. On this front, [BMSW18] provides a simple LP formulation for the revenue-maximizing auction for a single-buyer. We identify several formal barriers to extending this approach to multiple buyers.

==> MainBody/switching.tex <==
\begin{itemize}
    \item One result: recency bias doesn't fix FSE result.
    \item Conjecture? Switching regret doesn't fix FSE result either.
    \item Location of proofs: Shirley and Ben's final project, contained in Shirley's thesis.
    \item Todos: need to re go-over formal definitions, maybe modify definition of $\gamma$-mean based, dive into any challenges for switching regret. Chapter 5 of thesisformatted.
\end{itemize}
In this section we will attempt to extend the result of ~\cite{BravermanMSW18} in another direction: instead of considering multiple bidders, we will consider a single bidder who participates in the auction with a no regret algorithm that is not mean based. 

Recall that \cite{BravermanMSW18} presented a strategy for the seller such that when the bidder uses a mean-based no-regret strategy, the seller is able to extract revenue arbitrarily close to expected welfare. The strategy presented in the paper divides each arm $i$ (with label $w_i$) into the three following phases.

\begin{enumerate}
  \item $\emptyset$ session: $a_{t}(w_i) = 0$ and $p_t(w_i) = 0$, therefore the buyer never receives the item.
  \item $0$ session: $a_{t}(w_i) = 0$ and $p_t(w_i) = 1$, therefore the bidder always receives the item for price of $0$.
  \item $1$ session: $a_{t}(w_i) = 1$ and $p_t(w_i) = 1$, therefore the bidder always receives the item for price of $1$.
\end{enumerate}

We will investigate whether this construction still gives optimal revenue for bidding algorithms that are not mean-based. Specifically, we will consider two modifications to mean-based algorithms, recency bias and k-switching. We first consider when a bidder uses a mean-based algorithm with recency bias, weighting the rewards in each round by a factor more than the previous round. We also consider k-switching algorithms, where a mean-based algorithm receives all "meta-arms" that can switch items at most $k$ times. In both scenarios, we consider which values of parameters will allow the algorithm to remain no-regret if the original mean-based algorithm was no-regret. We then show that the example in \cite{BravermanMSW18} extracts maximum revenue from no-regret algorithms using recency bias, but the proof technique fails for algorithms with k-switching for any $k \ge 1$.

\subsection{Recency Bias}
\subsubsection{No-regret Recency Bias}
Consider a bidding algorithm $S^*$, such that the action on round $t+1$ given past rewards of $\{r_{w_i, s}(v_s)\}_{s \le t}$ will be the output of $S(\{\eta^sr_{w_i, s}(v_s)\}_{s \le t})$, where $S$ is a no-regret mean-based bidding algorithm. The first step is determining which values of $\eta$ will allow the algorithm $S^*$ to be no-regret given that $S$ was $\delta$-no-regret for some $\delta = o(T)$.

\begin{thm}
    If $S^*$ is an algorithm using a no-regret mean-based algorithm $S$ with recency bias factor $\eta > 1$, then $S^*$ is no-regret if $\eta$ satisfies $\eta^T \le 1 + \epsilon$ where $\epsilon$ is $o(1)$.
\end{thm}

\begin{proof}
    Let $b_t$ be the label of the arm the algorithm $S^*$ chooses in round $t$. $S$ is no-regret, which implies that for some $\delta = o(T)$, equation \ref{eq:1} below will hold.
    
    \begin{equation}
    E[\text{Regret}\Big(S(\{\eta^sr_{w_i, s}(v_s)\}_{s \le t})\Big)] = E\Big[\max_{i} \sum_{t=1}^T \eta^t r_{w_i, t}(v_t) - \sum_{t=1}^T \eta^t r_{b_t,t}(v_t) \Big]\le \delta
\label{eq:1}\end{equation}

This gives the following upper bound for the regret of $S^*$.

\begin{align*}
    E[\text{Regret}\Big(S^*(\{r_{w_i, s}(v_s)\}_{s \le t})\Big)] &= E\Big[\max_{i} \sum_{t=1}^T r_{w_i, t}(v_t) - \sum_{t=1}^T r_{b_t,t}(v_t) \Big] 
    \\ &\le E[\text{Regret}\Big(S(\{\eta^sr_{w_i, s}(v_s)\}_{s \le t})\Big)] + 2\sum_{t=1}^T (\eta^t - 1)
    \\ & \le \delta + 2T\epsilon := \delta^* = o(T)
\end{align*}

The first line is the definition of regret. The first inequality comes from the fact that $r_{w_i, t}(v_t) \le \eta^t - 1 + \eta^t r_{w_i, t}(v_t)$ for all $r_{w_i, t}(v_t) \in [-1,1]$, which is necessary to account for both positive and negative values of $r_{w_i, t}(v_t)$. Applying this inequality to each $r_{w_i, t}(v_t)$ term in the expression will give the resulting inequality by linearity of expectation. The second inequality is because $S$ is no-regret with parameter $\delta = o(1)$ and that by construction $\eta^t - 1 \le \eta^T - 1 = \epsilon = o(1)$. This shows that the expected regret of $S^*$ is upper bounded by $\delta^* = o(1)$, and therefore $S^*$ is a no-regret algorithm.
\end{proof}

The above theorem shows that $\eta^T \le 1 + \epsilon$ will preserve the no-regret property of the algorithm. Ideally, the restrictions on $\eta$ would be a function of $T$. The below lemma provides a slightly weaker condition on $\eta$, but one that is an explicit function of $T$.


\begin{lemma}
    If $\eta = 1 + \frac{\gamma}{T}$ where $\gamma = o(1)$, then $\eta^T = 1 + \epsilon$ for some $\epsilon = o(1)$
\end{lemma}
\begin{proof}
    $$\eta^T \le (e^{\frac{\gamma}{T}})^T = e^{\gamma} \le \frac{1}{1-\gamma} = 1 + \epsilon$$
    
    Where $\epsilon =\frac{1}{1 - \gamma} - 1$. Now we must show that $\epsilon = o(1)$. By definition, $\epsilon = o(1)$ if and only if $\frac{\epsilon}{1}$ goes to $0$ as $T$ goes to infinity.
    
    $$\lim_{T \to \infty} \frac{\epsilon}{1} = \lim_{T \to \infty} \epsilon = \lim_{T \to \infty} \frac{1}{1 - \gamma} - 1 = -1 + \lim_{T \to \infty} \sum_{i=0}^\infty \gamma^i = \lim_{T \to \infty} \sum_{i=1}^\infty \gamma^i = 0$$
    
    Where the last equality comes from the fact that $\gamma$ is $o(1)$ so $\lim_{T \to \infty} \gamma = 0$. Note we also used the fact that $\gamma < 1$, which is true for large enough $T$ because $\gamma = o(1)$.
\end{proof}

One question to consider is the tightness of the upper bound of $\eta^T \le 1 + \epsilon$ where $\epsilon = o(1)$. While we will not give a rigorous proof of the tightness, we will provide an example of how larger $\eta$ may pose problems. Suppose we have 

$$\eta = \exp\Big({\frac{\ln(T)}{T}}\Big) \approx 1 + \frac{\ln(T)}{T}$$

Consider a scenario where there is an arm $a$ that rewards $1$ for the first $\frac{T}{2}$ rounds and $0$ thereafter, and another arm $b$ that rewards $0$ for the first $\frac{3T}{4}$ rounds and rewards $1$ for the last $\frac{T}{4}$ rounds. In this case, a valid output by the no-regret algorithm $S$ with the $\eta$ scaled rewards as inputs would be to always pull arm $b$. This strategy would give regret for $S$ (as in Equation \ref{eq:1}) which is upper-bounded by $\max\Big({\frac{T}{2}\eta^{\frac{T}{2}} - \frac{T}{4}(\eta^{\frac{3T}{4}}),0}\Big)$. This value will be $0$ for large enough $T$, because $\eta^{\frac{T}{4}} \approx 1 + \frac{\ln(T)}{4} > 2$ for large enough $T$. This strategy, however, is not no-regret for the algorithm $S^*$. The regret for $S^*$ will be $\frac{T}{4} \ne o(T)$ and therefore $S^*$ will no longer be no-regret. In order to prove that $S^*$ is no-regret for larger values of $\eta$, proof techniques would most likely require more knowledge about the algorithm $S$ than just that it is no-regret.

\subsection{Multiplicative Weights}

Another way of obtaining the feasible values of $\eta$ that keep the algorithm no-regret is to plug $\eta$ directly into the upper bound for regret when using the Multiplicative Weights algorithm as described in \cite{arora2012multiplicative} for the mean-based no-regret algorithm $S$. The following upper bound comes from the analysis of the multiplicative weights algorithm. Note that in this expression, $\eta$ is once again the bias factor, $m^{(t)}$ is the costs of decisions in round $t$, $p^{(t)}$ is the distribution over decisions in round $t$, $n$ is the number of arms, and $\alpha$ is a positive constant of at most $\frac{1}{2}$.

$$\sum_{t=1}^T \eta^t m^{(t)} \dot p^{(t)}  - \sum_{t=1}^T \eta^t m_i^{(t)} \le  \alpha \sum_{t=1}^T \eta^t |m_i^{(t)}| + \frac{\ln(n)}{\alpha}$$

To get an upper bound on the regret for the algorithm $S^*$, we must derive an upper bound for the following expression without the scaling $\eta^t$ factors.

$$\sum_{t=1}^T m^{(t)} \dot p^{(t)}  - \sum_{t=1}^T m_i^{(t)}  $$

As in the theorem above, we will take $\eta$ such that $\eta^T = 1 + \epsilon$ with $\epsilon = o(1)$. By similar algebraic analysis to above, this gives the upper bound as follows.

\begin{align*}
    \sum_{t=1}^T m^{(t)} \dot p^{(t)}  - \sum_{t=1}^T m_i^{(t)} &\le \sum_{t=1}^T \eta^t m^{(t)} \dot p^{(t)}  - \sum_{t=1}^T \eta^t m_i^{(t)} + 2\sum_{t=1}^T (\eta^t -1)
    \\ &\le 2T\epsilon + \alpha\sum_{t=1}^T \eta^t + \frac{\ln(n)}{\alpha}
\end{align*} 

As in standard multiplicative weights, this is minimized at  $2\epsilon T + \sqrt{T\ln(n)} = o(1)$. In order to assure this is still $O(\sqrt{T\ln(n)})$, we must have $\epsilon = O(\frac{\ln(n)}{\sqrt{T}})$.

\subsubsection{Example Analysis}
\lindanote{TODO: define $A_j$, $B_j(v_i)$ again? Maye repeat the claim? }
Now, consider the proof of theorem B.1 in \cite{BravermanMSW18}. The proof relies on lemma B.2, which states that for each $w_i \in D$, and round $\tau \in [A_j, B_j(w_i)]$, $\sigma_{w_j,\tau}(w_i) > \sigma_{w_{j^{'}}, \tau}(w_i) + \gamma T$ for all $j^{'} > j$. We will show that an analagous theorem holds for algorithms using recency bias with appropriate $\eta$. 

\begin{lemma}
If $\eta^T = 1 + \epsilon$ where $\epsilon =o(1)$, then if the seller uses the example from \cite{BravermanMSW18}, for any $\tau \in [A_j, B_j^*(w_i)]$, where $B_j^*(w_i) := A_j + \frac{min(w_i,\rho)}{1-v_1}(1-\rho)(1-\delta)^{j-1}T - (\gamma + 2\epsilon)T$, the following holds:

\begin{equation}
\sum_{s=1}^\tau \eta^s r_{w_{j}, s}(w_i) - \sum_{s=1}^\tau \eta^s r_{w_{j^{'}}, s}(w_i) > \gamma T
\label{eq:2}\end{equation}

\end{lemma}

\begin{proof}


\begin{align*}
    \sum_{s=1}^\tau \eta^s r_{w_{j}, s}(w_i) - \sum_{s=1}^\tau \eta^s r_{w_{j^{'}}, s}(w_i) &\ge \sum_{s=1}^\tau r_{w_{j}, s}(w_i) - \sum_{s=1}^\tau r_{w_{j^{'}}, s}(w_i) - 2\sum_{s=1}^\tau (\eta^s - 1)
    \\& \ge \sum_{s=1}^\tau r_{w_{j}, s}(w_i) - \sum_{s=1}^\tau r_{w_{j^{'}}, s}(w_i) - 2\sum_{s=1}^T (\eta^s - 1)
    \\& \ge (\gamma + 2\epsilon) T - 2\epsilon T
    \\& = \gamma T
\end{align*}

The first inequality comes from the fact that $\eta^t r_{w_{j}, s}(w_i) \ge r_{w_{j}, s}(w_i) - (\eta^t - 1)$ and therefore this inequality can be applied to each term in the summation. The second inequality comes from the fact that all the terms in the summation are positive, so $\tau$ can be increased to $T$. The final inequality uses Lemma B.1 in \cite{BravermanMSW18}.
\end{proof}

Now, using the above lemma combined with the assumption that $S$ is $\gamma$ mean-based, the proof for theorem $B.1$ follows directly as in \cite{BravermanMSW18}.The only difference from the example in the paper is that we define $\gamma^* = \gamma  + 2\epsilon = o(1)$ and let

$$B_j^*(v) = A_j + \frac{min(v,\rho)}{1-v_1}(1-\rho)(1-\delta)^{j-1}T - \gamma^*T$$

The expected revenue of the seller when the bidder has value of $v_i$ must be at least

\begin{align*}
    q_i\sum_{j=1}^n(1-n\gamma)(B_j^*(v_i) - A_j(v_i)) &= q_i\sum_{j=1}^n (1-n\gamma)\Big( \frac{\min(v_i,\rho)}{1-v_1}(1-\rho)(1-\delta)^{j-1}T-\gamma^*T\Big)
    \\ &= (1-n\gamma)q_iT(-n\gamma^* + min(v_i,\rho)(1-(1-\delta)^n))
    \\ &\ge (1-\epsilon)q_iv_iT - o(T)
\end{align*}

The above equalities follow from the algebra in \cite{BravermanMSW18}. The rest of the proof then follows exactly as in \cite{BravermanMSW18} to show that revenue arbitrarily close to welfare is achieved. This means that recency bias with $\eta$ such that $\eta^T = 1 + o(1)$ does not break the example presented in \cite{BravermanMSW18}, and the seller is still able to extract $(1-\epsilon)Val(D) - o(T)$ revenue. 

This result can be generalized to a slightly wider range of $\epsilon$ with the following theorem. The proof is only outlined, but the general ideas are the same as in the proofs above.

\begin{thm}
    All mean-based algorithms with recency bias $S^*$ defined as $S^{*}(\{ r_{w_i, s}(v_s)\}_{s \le t}) = S(\{\eta^sr_{w_i, s}(v_s)\}_{s \le t})$ that satisfy $\sum_{t=1}^T \E\left[r_{w_i, t}(v_t)\right] - \sum_{t=1}^T \E\left[ r_{b_t,t}(v_t)\right] \le \sum_{t=1}^T \eta^t \E\left[r_{w_i, t}(v_t)\right] - \sum_{t=1}^T \eta^t \E\left[r_{b_t,t}(v_t)\right] + \beta T$ for any arm $i$ and strategy $b_t$ achievable by $S^*$ for some $\beta = o(1)$, are no-regret, Equation \ref{eq:2} holds, and Theorem B.1 in \cite{BravermanMSW18} is still valid.
\end{thm}
\begin{proof}
    The condition directly implies that $S^*$ is no-regret with $\delta^* = \delta + \beta T = o(T)$ where $\delta$ is the no-regret parameter in $S$. The algebra in Lemma 6 follows exactly the same in this case except with $\beta$ instead of $2\epsilon$, and the rest follows as above. 
\end{proof}

\subsection{k-switching}
\subsubsection{No-regret k-switching}
For k-switching, we will focus on bidders that use the multiplicative weights algorithm presented in \cite{arora2012multiplicative}. An algorithm $S^*$ with k-switching takes a no-regret mean-based algorithm $S$ (in this case multiplicative weights) and as input gives the set of meta-arms that consists of all strategies that switch arms at most $k$ times over the $T$ rounds. The following theorem illustrates for which values of $k$ the multiplicative weights algorithm remains no-regret.

\begin{thm}
    If $k = o(\frac{T}{\ln(T)})$, then the multiplicative weights algorithm with k-switching is no-regret.
\end{thm}
\begin{proof}
     The $k$ switching input to multiplicative weights has $n := \sum_{i = 0}^k m(m-1)^{i} \times {T \choose i} \le (Tm)^k$ arms that switch at most $k$ times. The regret bound in multiplicative weights gives the following upper bound on the regret where $i$ ranges over any $k$-switching arm and $Regret(i)$ is the regret with respect to arm $i$ \cite{arora2012multiplicative}.
    
    $$Regret(i) \le \eta \sum_{t=1}^T|m_{i}^{(t)}| + \frac{\ln(n)}{\eta}$$
    
    Because switching $0$ times is a meta-arm in k-switching, the regret with respect to any 0-switching arm also obeys this upper bound. Substituting the upper bound for $n$ and the upper bound $|m_{i}^{(t)}| \le 1$ gives an upper bound on the regret of 
    
    $$Regret(i) \le \eta T + \frac{k\ln(Tm)}{\eta}$$
    
    This is minimized for $\eta = \sqrt{\frac{k\ln(Tm)}{T}}$ with value $\sqrt{Tk\ln(Tm)}$. Simple algebra gives that this upper bound is $o(T)$ when $k = o(\frac{T}{\ln(T)}$).

\end{proof}

Clearly, the maximum number of switches is $T-1$, and the above theorem shows that $k = o(\frac{T}{\ln(T)})$ will keep the algorithm no-regret, therefore allowing close to the maximal number of switches, despite the number of arms growing exponentially with $k$.


\subsubsection{Example Analysis}
Let $M(i,j,t)$ be the label of the meta-arm that switches from arm $i$ to arm $j$ at time $t$ and let $M(j)$ be the label of the arm $j$ with no switches. The example as presented in Theorem B.1 in \cite{BravermanMSW18} encounters problems for mean-based no-regret algorithms that use k-switching for any $o(\frac{T}{\ln(t)}) \ge k \ge 1$, which by the above theorem are still no-regret. We will explore in further detail the case when $k = 1$, as even this value of $k$ will invalidate the proof. The first problem that arises is that the proof relies on Lemma B.2 to show that any mean-based algorithm with value $w_i$ will choose any arm $l > j$ for any round in the interval $[A_j,B_j(w_i)]$ with probability at most $\gamma$. Lemma B.2 shows that the utility from arm $j$ will be larger than the utility for any arm $l > j$ by at least $\gamma T$, and because the algorithm is mean-based, this implies that arm $l$ will be chosen with probability at most $\gamma$. Unfortunately, with $k$-switching, the meta-arm $M(j)$ no longer serves the purpose of showing that any arm $l > j$ will be chosen with probability at most $\gamma$. To see this, consider the meta-arm $M(j,n,A_j)$, that is the meta-arm which chooses arm $j$ up until arm $j$ starts charging $1$, and then switches to the last arm. By construction, for $\tau \ge A_j + \frac{\gamma}{1-w_i}T$

    $$\sigma_{M(j,n,A_j),\tau}(w_i) \ge \sigma_{M(j),\tau}(w_i) + \gamma T.$$

But $M(j,n,A_j)$ will choose arm $n > j$ in round $\tau$, invalidating the proof in \cite{BravermanMSW18}. Fortunately, we can actually show that by looking at a different meta-arm, a variant of Lemma B.2 will hold. 

\begin{lemma}
    If the buyer has value $w_i$, then for any $\tau \in [A_j,B_j(w_i)]$, any meta-arm that chooses arm $l > j$ in round $\tau$ will be chosen by the algorithm with probability at most $\gamma$.
\end{lemma}

\begin{proof}
    Consider the meta-arm $M(1,j,A_1)$. This arm always has as much historical reward as arm $M(j)$, therefore by lemma B.2, $\sigma_{M(1,j,A_1), \tau}(w_i) \ge \sigma_{M(k), \tau}(w_i) + \gamma T$ for $k > j$. Furthermore, $\sigma_{M(1,j,A_1), r}(w_i) \ge \sigma_{M(k,l,t), \tau}(w_i) + \gamma T$ for any $k,l > j$. Now, the only arms left to consider are those of the form $M(k,l,t), r$ where $t \le \tau$, $k \le j$, and $l > j$. By construction, the best such arms are of the form $M(k,l,A_k)$, in other words switching right after the $0$ period ends on arm $k$. By lemma B.2 in \cite{BravermanMSW18}, arm $j$ between rounds $A_1$ and $\tau$ will have at least $\gamma T$ more total reward than arm $l > k$  between rounds $A_k$ and $\tau$, as these intervals cover the entire ranges that arms $j$ or $l$ sell the item. Furthermore, arm $1$ has the longest $0$ period, therefore arm $1$ between the first round and round $A_1$ will have at least as much total reward as arm $k$ between the first round and round $A_k$. Combining these previously two statements gives that $\sigma_{M(1,j,A_1), \tau}(w_i) \ge \sigma_{M(k,l,A_k), \tau}(w_i) + \gamma T$. Therefore, $\sigma_{M(1,j,A_1), \tau}(w_i)$ has at least $\gamma T$ more total reward that any meta-arm that chooses arm $l > j$ in round $\tau$, and therefore the mean-based algorithm will choose any meta-arm that chooses arm $l > j$ in round $\tau$ with probability at most $\gamma$.
\end{proof}

Unfortunately, this is where we encounter another hurdle. Above, we showed that a meta-arm that chooses arm $l > j$ at round $\tau$ will be pulled with probability at most $\gamma$, but unfortunately we can no longer take a union bound over all $n$ arms and state that the probability that any arm $l > j$ is chosen with probability at most $n\gamma$. We now have $\approx Tm^2$ meta-arms in the algorithm, therefore the union bound gives that an arm $\le j$ will be chosen in round $\tau$ with probability at least $1-Tm^2\gamma$. Unfortunately, if $\gamma = o(1)$, then it is possible for $1-Tm^2\gamma < 0$, and therefore the union bound is not useful. One potential solution would be to enforce the algorithm being used by the bidder to be $\gamma$-mean based for $\gamma = o(\frac{1}{T})$, as this would allow the union bound to hold and give the expected revenue of the seller the same as in the proof of Theorem B.1.
